A Digital Twin Description Framework and its Mapping to Asset Administration Shell

The pace of reporting on Digital Twin (DT) projects continues to accelerate both in industry and academia. However, these experience reports often leave out essential characteristics of the DT, such as the scope of the system-under-study, the insights and actions enabled, and the time-scale of processing. A lack of these details could therefore hamper both understanding of these DTs and development of DT tools and techniques. Our previous work developed a DT description framework with fourteen characteristics as a checklist for experience report authors to better describe the capabilities of their DT projects. This report provides an extended example of reporting to highlight the utility of this description framework, focusing on the DT of an industrial drilling machine. Furthermore, we provide a mapping from our description framework to the Asset Administration Shell (AAS) which is an emerging standard for Industry 4.0 system integration. This mapping aids practitioners in understanding how our description framework relates to AAS, potentially aiding in description or implementation activities.

==> sections/background.tex <==
\section{Background on Digital Twins}
\label{sec:background}









==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}


In this section, we evaluate our presented approach by performing case studies. %, following the guidelines by Runeson and Höst~\cite{Wohlin2012}. \bentley{Javier, is this citation correct?} \javier{Not totally sure if we do as they recommend. In any case, we can place this reference in the threats to validity}


\subsection{Research Questions}\label{sec:RQs}

Our main interest is in realizing whether techniques of symbolic-execution and SBFL can be combined together to effectively and efficiently identify faulty rules in model transformations. We therefore aim to answer the following research questions (RQs):

%\newcommand{\RQOne}{\emph{Can SBFL be used to effectively detect bugs in model transformation verification?}} 


%\newcommand{\RQOneOne}{\emph{Are there techniques that allow us to quickly find the faulty rule?}}

%\newcommand{\RQOneTwo}{\emph{Amongst those techniques, are there techniques that are best in most cases?}}

%\newcommand{\RQTwo}{\emph{Is it possible to automate the process of locating faults in model transformation verification applying spectrum-based techniques?}}

\begin{itemize}
    \item \textit{RQ1 - How can the techniques of symbolic-execution and SBFL be combined together to automatically identify faulty rules in a transformation?}
    \item \textit{RQ2 - Is the resulting approach powerful enough to discover faulty rules effectively?}
    \item \textit{RQ3 - Is there a difference in effectiveness of applying the different SBFL techniques for fault localization in model transformation?}
    \item \textit{RQ4 - Is the resulting approach fast enough to discover faulty rules efficiently?}
\end{itemize}

%Many techniques for suspiciousness computation have been proposed in the literature in different fields, and we want to determine whether there are techniques that allow us to quickly find the faulty rule in our context, answering RQ1.1. 
%Amongst those techniques, we want to determine which ones are best in most cases, answering RQ1.2.
%Finally, since there has been no proposal so far for the application of SBFL techniques for locating faults in MT verification, we want to determine whether it is feasible to develop an automated approach, answering RQ2.

\subsection{Experimental Setup}\label{sec:ev_setup}

This section will briefly describe our experimental setup, including the description of our case studies and the SBFL techniques under study.

\subsubsection{Case Studies}\label{sec:case_studies}

Two case studies have been used in the evaluation of our technique. The first case study is the \FTP transformation, which was translated automatically from the Atlas Transformation Language (ATL)~\cite{atlTool} and expanded upon in previous verification work~\cite{Oakes2015, Oakes2016}. This transformation has also been discussed in related verification and testing research~\cite{Gogolla2011}.

This transformation is composed of 19 rules, and takes \textit{Families} of \textit{Members} who live in \textit{Countries} and \textit{Cities}, and converts those elements into \textit{Men} and \textit{Women} who live in \textit{Communities} and work at \textit{TownHalls}. For brevity, we omit figures and descriptions for the input and output meta-models here, as they can be found in Oakes \textit{et al.}~\cite{Oakes2016}.

The second case study is the \UMLER transformation containing 9 rules, taken from~\cite{Burgueno2015}. Note that the \UMLER transformation has previously been studied in the context of SBFL in~\cite{TroyaSBFL18}.

Two sets of contracts for the \FTP transformation have been employed. The first set is the contracts found in the thesis of Oakes~\cite{Oakes2018}, where the contracts are expected to hold in all transformation executions (so-called `positive' contracts).  As an example, the \textit{Pos\_FourMembers} contract is displayed in Figure~\ref{fig:fourMembers_intro} on page~\pageref{fig:fourMembers_intro}.
The second set of contracts for the \FTP transformation have been created for this work, and are derived from the rules of the correct transformation\footnote{The contract which is a mirror of the \textit{acommitteeSolveRefCompanyCityAssociationCommittee} rule was excluded, because it was not holding in every path condition for the transformation.}.

% A selection of these contracts are briefly summarized in Table~\ref{tab:ftp_contracts} to indicate their involved elements and intention, and

% \begin{table}[tbp]
%     \centering
%     \begin{tabular}{l|p{5.2cm}}
%         \textbf{Contract Name} & \textbf{Description} \\\hline
%         Pos\_FourMembers & Are two \textit{Men} and two \textit{Women} created from a \textit{Family} of four \textit{Members}?\\
%         Pos\_MotherFather & Are \textit{Man} and \textit{Woman} elements created with their correct \textit{fullName} attribute?\\
%         Pos\_AssocCity & Do \textit{Community}, \textit{City}, and \textit{Company} elements correctly produce a \textit{Community} with a \textit{TownHall} and a \textit{Committee}?\\
%         Pos\_ChildSchool & If a \textit{Child} \textit{goesTo} a \textit{School} that has a special \textit{Service}, is a \textit{SpecialFacility} created with a \textit{Person} as a\textit{member}?\\\hline
%         Neg\_SchoolOrdFac & Is a \textit{OrdinaryFacility} always created from a \textit{School}?\\
%         Neg\_DaughterMother & Is a \textit{Man} always produced from a \textit{Family} including a daughter and a mother?\\
%     \end{tabular}
%     \caption{\FTP contracts, including two contracts expected to fail for some rule combinations.}
%     \label{tab:ftp_contracts}
% \end{table}

Note that the former contracts rely on the output of the execution of multiple rules, while the latter contracts focus on the execution of a single rule. As such, the former can be viewed as `integration-test' contracts, while the latter are `unit-test' contracts. %It is our hypothesis that `unit-test' contracts are more suited to detect errors when the transformation is mutated. This hypothesis is further discussed in Section~\ref{sec:unit-integration-contracts}.

For the \UMLER contracts, we adapted the contracts found in~\cite{TroyaSBFL18}. Note that the contracts in that work operate on models with instantiated elements. In contrast, the contracts in symbolic-execution verification operate on an abstracted representation of the transformation, where it is unknown how many times a particular rule has executed. Further details on the implications of this abstraction are found in the thesis of Oakes~\cite{Oakes2018}.


% \subsubsection{Test suite}\label{sec:test_suite}
% Do we need a test suite at all? We can maybe show the different path conditions we get. 

\subsubsection{Generating Mutants}\label{sec:mutants_eval}

 For evaluating our approach, we require a set of transformation rules with known induced faults. To support this, we have implemented automatic mutation of DSLTrans transformations. 
 Table~\ref{tab:mutations} shows the set of implemented mutations along with a brief description. %Future work will expand these mutations to capture more possible transformation errors.
 
 \begin{table}[tbp]
    \centering
    \caption{Set of mutations implemented.}
    \label{tab:mutations}
    \begin{tabular}{@{}lp{5cm}@{}}
        \textbf{Mutation Name} & \textbf{Description} \\\toprule
        Add Class & Adds a random class from the input or output meta-model\\
        Add Association & Adds a valid association between two classes (if not existing)\\
        Add Backward Link & Adds backward link (see Section~\ref{sec:dsltrans})\\\midrule
        
        Delete Element & Deletes an association or class (and connected assocs.)\\
        Delete Equation & Deletes an equation (for matching or setting attribute values)\\\midrule
        
        Retype Class & Replaces a class's type by a type up or down the inheritance hierarchy\\
        Retype Assoc. & Replaces an association's type by another valid association\\\midrule
        
        Modify Equation & Replaces part of an equation, such as removing terms in a concatenation, or changing involved attributes\\\bottomrule
    \end{tabular}
    
\end{table}

As an example, consider the DSLTrans rule presented in Figure~\ref{fig:DSLTrans_rule_back} on page~\pageref{fig:DSLTrans_rule_back}. This rule has 49 mutations applied to it in our current framework: 23 \textit{Add Class} mutations, 3 \textit{Add Association}, 4 \textit{Add Backward Link}, 10 \textit{Delete Element}, 3 \textit{Retype Class}, and 6 \textit{Retype Assoc.} 
 
 These mutations are applied to all rules in the \FTP and \UMLER transformations, generating 931 and 191 mutants, respectively. Each mutant is fed as input to the SyVOLT transformation verifier, along with the contracts for the case study.
 
\begin{table}[tbp]
\caption{Suspiciousness computation techniques.}
  \label{tab:techniques}
  \centering
\begin{tabular}{l}
\toprule
    \textbf{Technique} \textbf{and} \textbf{Formula} \\
\midrule
\rule{0pt}{3ex} Barinel~\cite{AbreuZG09}: \multicolumn{1}{c}{ \scriptsize$1 - N_{CS} / (N_{CS}+N_{CF})$} \\[2ex] \hline
\rule{0pt}{3ex} Braun-Banquet~\cite{WongGLAW16}:  \multicolumn{1}{c}{ \scriptsize$N_{CF} / max(N_{CF}+N_{CS}, N_{CF}+N_{UF})$ }\\[2ex] \hline
\rule{0pt}{3ex} Kulczynski2~\cite{NaishLR11} : \\  \multicolumn{1}{c}{ \scriptsize$0.5 \times \big(N_{CF} / (N_{CF}+N_{UF}) + N_{CF} /(N_{CF}+N_{CS}) \big)$}\\[2ex] \hline
\rule{0pt}{3ex} Mountford~\cite{WongDLG12} :  \\ & \multicolumn{1}{c}{ \scriptsize $N_{CF} /$ $\big(0.5\times \big((N_{CF}\times N_{CS})+(N_{CF}\times N_{UF})\big) +  (N_{CS}\times N_{UF})\big)$} \\[2ex] \hline
\rule{0pt}{3ex} Ochiai~\cite{AbreuZGG09} : \multicolumn{1}{c}{ \scriptsize$N_{CF} / \sqrt{N_F\times(N_{CF}+N_{CS})}$}\\[3ex] \hline
\rule{0pt}{3ex} Ochiai2~\cite{AssiriYB2017} : \multicolumn{1}{c}{\scriptsize ($N_{CF}\times N_{US}) / $}\\ & \scriptsize $\sqrt{(N_{CF}+N_{CS})\times (N_{US}+N_{UF})\times(N_{CF}+N_{UF})\times(N_{CS}+N_{US})}$ \\[2ex] \hline
\rule{0pt}{3ex} Op2~\cite{NaishLR11}  : \multicolumn{1}{c}{ \scriptsize$N_{CF} - N_{CS} / (N_{S}+1)$} \\[2ex] \hline
\rule{0pt}{3ex} Phi~\cite{MaxwellP68}  : \multicolumn{1}{c}{ \scriptsize$(N_{CF}\times N_{US}-N_{UF}\times N_{CS}) / $ } \\ & \multicolumn{1}{c}{\scriptsize $\sqrt{(N_{CF}+N_{CS})\times (N_{CF}+N_{UF})\times (N_{CS}+N_{US})\times (N_{UF}+N_{US})}$ }\\[2ex] \hline
\rule{0pt}{3ex} Tarantula~\cite{JonesH05} : \multicolumn{1}{c}{ \scriptsize $(N_{CF}/N_{F})/\big((N_{CF}/N_F)+(N_{CS}/N_S)\big)$ }\\[2.5ex] \hline
\rule{0pt}{3ex} Zoltar~\cite{JanssenAvA09} : \\ \multicolumn{1}{c}{\scriptsize $N_{CF} / \big(N_{CF}+N_{UF}+N_{CS}+(10000\times N_{UF}\times N_{CS})/N_{CF}\big)$ }\\[3ex]
\bottomrule
\end{tabular}
\end{table}

\input{evaluation/metrics-average.tex}
 
 
\subsubsection{Techniques for Suspiciousness Computation}\label{sec:techniques}
There are several techniques proposed in the literature for suspiciousness computation. We want to study how effective they are in the context of model transformation verification, i.e., how helpful they are in finding the faulty transformation rule. For this, we have surveyed papers that apply SBFL in different contexts and have selected ten techniques. They are displayed with their corresponding suspiciousness computation formulae in Table~\ref{tab:techniques}.

\emph{Tarantula}~\cite{JonesH05} is one of the best-known fault localization techniques.
It follows the intuition that statements that are executed primarily by more failed test cases are highly likely to be faulty.
Additionally, statements that are executed primarily by more successful test cases are less likely to be faulty.
The \emph{Ochiai} similarity coefficient is known from the biology domain and it has been proved to outperform several other coefficients used in fault localization and data clustering~\cite{AbreuZGG09}.
This can be attributed to the Ochiai coefficient being more sensitive to activity of potential fault locations in failed runs than to activity in passed runs.
\emph{Ochiai2} is an extension of this technique~\cite{NaishLR11,WongGLAW16,AssiriYB2017}.
\emph{Kulczynski2}, taken from the field of artificial intelligence, has showed promising results in preliminary experiments, and \emph{Phi} and \emph{Op2} have been considered in some comparative studies with other metrics~\cite{NaishLR11,XieCKC13,WongGLAW16}.
The framework called \emph{Barinel}~\cite{LuciaLJTB14} combines spectrum-based fault localization and model-based debugging to localize single and multiple bugs in programs. 
\emph{Zoltar}~\cite{JanssenAvA09} is also a tool set for fault localization.
\emph{Mountford} behaves as the second best technique, among 17 of them, for a specific program in a study performed in~\cite{WongDLG12}.

\subsection{Experimental Results}\label{sec:ev_results}


\input{evaluation/bc_wc_diff.tex}

As explained in Section~\ref{sec:sbfl-background}, there can be ties in the suspiciousness-based rankings. This is the reason why the EXAM scores (cf. Section~\ref{sec:suspiciousness}) for the best-, worst- and average-case scenarios need to be obtained. Table~\ref{tab:avg_score} displays the average results given by our approach with the ten implemented techniques in the \textbf{average-case scenario}. The table shows the mean, median and standard deviation of the EXAM scores of each case study.

%Recall that, in our context, the EXAM score represents the percentage of rules that have to be examined until the faulty rule is located. In the \UMLER case study, since we have 9 rules, the lowest value of the EXAM score is $\frac{1}{9}=0.\wideparen{1}$, which means that the faulty rule is placed first in the suspiciousness-based ranking. In the \FTP case study, we have 19 rules, so the lowest value for the EXAM score is $\frac{1}{19}=0.053$.

As we have explained in Section~\ref{sec:sbfl-background}, the lower the EXAM score, the better. We consider that having an EXAM score below 0.3 is acceptable. 
%In the \UMLER case study, this means we have to inspect up to 2.7 rules until we find the faulty one. In the \FTP case study, an EXAM score below 0.3 means we have to inspect 5.7 rules in order to locate the faulty rule. 
In Table~\ref{tab:avg_score}, we have highlighted with bold font those EXAM scores whose mean is below 0.3. We have grouped the results by case study, and the last block shows the average values.

We can see that the different techniques behave similarly in all case studies. We see that \emph{Braun-Banquet}, \emph{Kulcynski2}, \emph{Mountford}, \emph{Ochiai}, \emph{Op2} and \emph{Zoltar} provide the best results (i.e., the lowest EXAM scores). Among them, we can leave out \emph{Mountford} and \emph{Braun-Banquet}, since they provide an EXAM score above 0.3 for at least one case study. For the other four techniques, we can see that the median and standard deviation values are very similar for all of them in each case study.  Having a look at the overall values, we see that \emph{Kulcynski2} and \emph{Zoltar} give the best results, i.e., the lowest mean for the EXAM score, being the median and standard deviation the same. They are closely followed by \emph{Ochiai}, and we have \emph{Op2} in the fourth position. These four techniques result in an EXAM score below 0.25.

In this section we have focused on the average-case scenario values so far. For having an idea about the number of ties in the different suspiciousness-based rankings, Table~\ref{tab:bc_wc_diff} displays the average values for the mean of the EXAM score in the best- and worst-case scenarios for all case studies. It also shows the absolute value of the difference between both values (column \emph{Diff}). In some techniques, we can deduce there are a large number of ties. For instance, the difference of the EXAM scores between best- and worst-case scenarios for the \emph{Barinel} and \emph{Tarantula} techniques are 0.633, 0.597 and 0.445, where the average of 0.558 is quite high. Interestingly, the four techniques that gave the lowest EXAM scores in the average-case scenario (cf. Table~\ref{tab:avg_score}) also seem to have the lowest number of ties, since their differences in the EXAM scores in the best- and worst-case scenarios are the lowest among all ten techniques. In fact, the average difference for the \emph{Op2} technique is 0.196, and for \emph{Kulcynski2}, \emph{Ochiai} and \emph{Zoltar} the value is 0.217.
 
 
\subsection{Discussion}\label{sec:discussion}
This section provides a short discussion about the research questions we identified.

\subsubsection{RQ1 - Automation}\label{sec:RQ1}

To address this RQ, we have built a script to coordinate the mutation and verification processes. The output provided by this step, numbered as Step 2 in Figure~\ref{fig:methodology}, is the input for the SBFL process. The latter produces a set of comma-separated value (csv) files providing the suspiciousness-based rankings whenever a contract fails. It also provides the EXAM scores for each ranking, values that we have used in this evaluation. All these artifacts are available on our online materials~\cite{SyVOLTSBFL18-online}. We thus answer in the affirmative, in that this approach can be and has been automated.

\subsubsection{RQ2 and RQ3 - Effectiveness}\label{sec:RQ2}

The results in Section~\ref{sec:ev_results} show the comparison between different state-of-the-art techniques for suspiciousness computation on our case studies.
As we see in Table~\ref{tab:avg_score}, there is considerable variation between the techniques. For instance, there are techniques that provide an average EXAM score in the average-case scenario nearly to or even above 0.5, such as \emhp{Barinel}, \emph{Ochiai2}, and \emph{Phi}. We can say these techniques are not effective, since their effectiveness is the same as if the suspiciousness rankings were created randomly. 

However, there are techniques that can be considered indeed effective in our context. As discussed in Section~\ref{sec:ev_results}, the most effective techniques are, in this order,  \emph{Kulcynski2}, \emph{Zoltar}, \emph{Ochiai}, and \emph{Op2}. For all of them, the average EXAM score considering all case studies is below 0.25, meaning that we need to inspect less than a quarter of the transformation in order to find the faulty rule. Furthermore, studying Table~\ref{tab:bc_wc_diff}, we concluded that these four techniques do not compute a large number of ties in the suspiciousness-based rankings, meaning they are able to clearly identify and position the faulty rules among the first ones in the ranking.

As an answer for RQ2 and RQ3, we conclude that our approach is powerful enough to discover faulty rules effectively, and the four techniques in the previous paragraph are the most effective ones. In fact, in the UML2ER case study, also studied in~\cite{TroyaSBFL18}, we get EXAM scores below 0.3 with these techniques, while Troya et al.~\cite{TroyaSBFL18} report only values above 0.3.

\subsubsection{RQ4 - Performance}
 The focus of the current paper is on the application of the SBFL technique to symbolic-execution transformation verification. As such, our focus was not on rigorously measuring or optimizing execution times or other resource consumption.
 As a rough guide, the SyVOLT tool takes around two seconds on the authors' laptop to produce verification output for each mutant. Thus verification of all mutants takes around 30 minutes for the 931 mutants of the \FTP transformation and 7 minutes for the 191 mutants of the \UMLER transformation. Suspiciousness values are then computed in less than 10 seconds for \UMLER and less than 1 minute for \FTP.
 
We conclude that for transformations of this size, this is a reasonably efficient process. Future work will study the scalability of this approach and consider improvements.



%\subsubsection{Unit-test versus Integration Contracts}
%\label{sec:unit-integration-contracts}
%We note that the unit tests are different than the integration tests in that...
%\javier{let's see whether to keep this here or explaining in the discussion}
  
\subsection{Threats to Validity}\label{sec:ev_threats}
Wohlin et al.~\cite{Wohlin2012} identify four types of threats that can affect the validity of our study.

\subsubsection{Conclusion Validity} The first threat is drawing incorrect conclusions from the experimental data. To mitigate this, we have applied statistical analysis by comparing the mean, median and standard-deviation of all case studies, and also considering the differences in the EXAM scores of best- and worst-case scenarios. 

\subsubsection{Construct Validity} A possible construct validity threat is the use of one single metric, the so-called EXAM score, to evaluate the effectiveness of the different techniques. Other metrics have been proposed~\cite{WongGLAW16}, such as the T-score~\cite{Liu06}, P-score~\cite{ZHANG20091573} and N-score~\cite{Gong12}.
However, the EXAM score is an accepted metric for measuring the quality of SBFL techniques, and has been used in a variety of works~\cite{WongGLAW16}.
% Moreover, we have decided to obtain the EXAM score as it is directly applicable in the context of model transformation verification.
By considering the transformation rules as units of examination, the EXAM score is easy to obtain and understandable, since it is directly proportional to the amount of rules to be examined.
% , rather than to an indirect measurement in terms of the amount of code that does not need to be examined, as proposed by other scores.

\subsubsection{Internal and External Validity} These threats are those factors that might affect the results of our evaluation, and our ability to generalize our results.

We have tried to minimize these threats by selecting a case study, \UMLER, that has been used in previous work for locating faults in model transformations~\cite{Burgueno15,TroyaSBFL18}. This is complemented with the larger \FTP case study. The union of both case studies considers most DSLTrans constructs, and both case studies differ in their domains, size of metamodels and transformation. In any case, we leave the examination of more case studies for future work.

As well, we have constructed a set of contracts that cover much of the specifications of the transformations. In total, we have 35 contracts (13 in \UMLER, 16 unit-test and 6 integration-test contracts in \FTP). 
For the \UMLER case study, we have taken the contracts proposed in~\cite{Burgueno15} and also used by~\cite{TroyaSBFL18}.

We have also tried to create a large set of 1122 mutants (931 in \FTP and 191 in \UMLER), and we have aimed at maximizing the variation of semantic faults and mutation operators used. However, we acknowledge that different mutation operators could have an impact on the results.

Finally, we have implemented our approach for DSLTrans and SyVOLT since they provide a powerful tool-set for the application of symbolic-execution transformation verification. However, we do believe our approach would produce similar results for any model transformation verification language and tool that provides the same analysis possibilities and outputs. Any such tool may serve as input for our SBFL computation (cf. steps 2 and 3 in Figure~\ref{fig:methodology}), which constructs the coverage matrices and error vectors, and computes the suspiciousness-based rankings.

%Limitations of DSLTrans -
%Restricted because of confluence, termination
%No deletion, loops, best suited for translation transformations
%Can use other transformation languages, but need symbolic execution for them

%Limitations of SyVOLT - 
%Uses abstraction over multiplicity, means loss of information
%General lack of verification potential compared to instance-based approaches
%Limited contract language

%\subsubsection{Not-Applicable Results}
%\label{sec:not-applicable}
%PCs being Not Applicable to Contracts -
%N/A results don't give much information
%When mutating, all contracts tend to fail or succeed. How to beat this?

%How to develop contracts (integration/unit-test)? - 
%Does integration or unit-test work better?
%Developing contracts is larger verification work question

%How to choose best suspiciousness technique?

%Only two case studies -
%In future can do more


==> sections/further_example_table.tex <==
{ 

\tymin=35pt

%\begin{landscape}
	\begin{table*}[tbp]
		\scriptsize
		\caption{Four digital twin experience reports as presented in our conceptual structure.}
		\label{tab:further_examples}
\begin{tabulary}{\textwidth}{L||L|L|L|L}%|L|L|L|L}
	
\toprule
Expr. Report &
Boat Avatar~\cite{Wuest2015} &
Cyber Guided Vehicle~\cite{Bottani2017} &
%Wind Turbine Gearbox~\cite{Tao2018a} &
Oil and Gas Drilling~\cite{Mayani2018} &
Petrochemical Optimization~\cite{Min2019}\\\midrule\midrule
System-under-study &
\textit{Leisure boats and stakeholders (owners, manufacturers, social networks) (?).} &
Auto. guided vehicle (AGV) in job-shop prod. system. &
Performance of and forces on drilling rig. &
%Turbine gearbox stresses and wear. &
Catalytic cracking unit in petrochemical production line.\\\midrule
Multipl. &
DT instances per boat. &
DT instances per prod. system. &
DT instances per drill site. &
%DT instances per wind turbine. &
DT instances per unit.\\\midrule
Usages &
Optimizing design/production, enhancing boat experience, upgrade services. &
Optimizing policy for system profit, visualization. &
Planning, training, operation forecasting. &
%Health management. &
Production optimization.\\\midrule
Enablers &
Production decision support, web presence, maintenance recommenders. &
Simulator, AGV controller. &
Sim. of performance and forces, auto. monitoring.&
\textit{``Profit and market modelling systems'', ``sim. and opt. systems'', machine-learning algs.}
%Simulator and machine learning component. &
\\\midrule
Models \& Data &
Data from boat, predictive models for maintenance recommenders. &
Model of shop, AGV code, prod. data. &
Sensor data, hydraulic and mechanical models. &
Machine learning models, historic data.%Component models, vibration data, neural network. &
\\\midrule
Slices &
[Omitted for space] &
Same slice for usages. &
[Omitted for space] &
\textit{Unclear.}
%Only one slice. &
\\\midrule
Fidelity Consid. &
\textit{Realistic for optimizing and services, less realistic for boat experience. Not explicit.}&
\textit{Realistic for optimization, less realistic for viz. Not explicit.}&
\textit{Highly realistic for planning and forecasting, realistic for training. Not explicit.} & Realistic. Data must be cleaned and aligned before processing.
%Highly realistic. &
\\\midrule
Data Comm. &
Auto: Assorted boat conditions, such as battery/fuel level, current weather, maintenance status, position, etc. &
\textit{None (possibly code?).} &
%Auto: Vibration, speed, power output. &
Auto: Temperature, pressure, etc. &
Production plans, production line data.\\\midrule
Ins. \& Act. &
\textit{I: Boat info., service recommendations \& offers. A: Posting to social networks(?).} &
\textit{I/A(?): AGV controller code.} &
%I: Maintenance strategies. &
I: Performance reports. A: Drill control signals. &
\textit{I: "Analysis data" and recommendation info.  A: Control instructions.}
\\\midrule
Time-Scale &
\textit{Slower-t-r-t insights, real-time data, real-time posting to social networks (?).} &
Slower-t-r-t. &
%Slower-t-r-t for health data reports for maintenance insights, real-time data. &
\textit{Slower-t-r-t for reports \& training, real-time for control, faster-t-r-t for sim.(?).} &
Slower-t-r-t historical data and insights, real-time data and control actions.\\\midrule
Acting Compon. &
Created web platform integration. &
\textbf{No compon. additions reported.} &
%None (no actions). &
\textbf{No compon. additions reported.} &
\textit{``Industrial IoT systems'', such as ``electric and electronic circuits''}
\\\midrule
Sensing Compon. &
Product Life-cycle Management system, data integration layer&
\textbf{No compon. additions reported.} &
%\textbf{No compon. additions reported.}&
\textbf{No compon. additions reported.} &
Measuring instruments, ``sampling, preprocessing and injection systems'', monitors and recorders.
\\\midrule
Life-cycle Stages &
\textit{Ideation, realization, utilization, reclamation. SUS: No manufacturers in middle stages (?).} &
Utilization. &
%Utilization. &
Ideation, realization, utilization. &
Utilization. \\\midrule
Evolution &
Usages created, then data connection, then insight/action connection. &
\textbf{Not reported.} &
%\textbf{Not reported.} &
\textit{Used for training, then used for control(?).} &
Basic DT constructed, then trained on existing data, then connected to SUS.\\\midrule\midrule
Class. &
DS/DT (?) &
DS/DT (?)  (versus DT by~\cite{Kritzinger2018}) &
DT &
DT (versus DS by~\cite{Fuller2019})\\
\bottomrule
\end{tabulary}





%
%
%~\\~\\
%
%
%
%
%
%
%\begin{tabulary}{\textwidth}{L||L|L|L}\toprule
%
%\textbf{Case Study}         & \textbf{Air Force~\cite{Tuegel2011}}                            & \textbf{Wind Turbine~\cite{Tao2018a}}                                                                       & \textbf{Drilling \cite{Mayani2018}}        \\\midrule\midrule%                                         & \textbf{Nautical Thrusters~\cite{Ludvigsen2016}}                                                                                                                             & \textbf{Boat Avatar~\cite{Wuest2015}}                                                                                                                                                                                                           & \textbf{Optimization~\cite{Guerra2019}}                                                                        & \textbf{Prod. Sys.~\cite{Uhlemann2017}}                                                                                                                                                                        
%
%
%\textbf{System-under-study}
% & Aircraft, mechanical stresses on materials                                                                                                                                                                            & WT gearbox stresses and wear
% & Performance of and forces on drilling rig
%\\\midrule
%%& Vessel control systems and environment
%%& Product Avatar, Leasure boat avatar                                                                                                                                                                                    & Ultraprecision motion system with backlash and friction                                & Production systems, logistics, industry 4.0 in SMEs                                                                                                                                   \\
%\textbf{Multipl.}          & One DT per aircraft                                                                                                                                                                                                                       & One DT per WT
% & One per drill site
%\\\midrule
%%                                   & one for a generic instance                                                                                                                             & One DT per boat                                                                                                                                                                                                        & One DT representing a generic instance                                                 & Unclear                                                                                                                                                                               
%%\textbf{Usages}                  & Maintenance forecast, damage prediction                                                                                                                                                                                                        & Health management                                                      & Planning, training, operation forecasting                 & Control system verification                                                                                                                            & Enhancing experience, Storage monitoring, EOL services, Refurbishment, maintenance                                                                                                                                     & Optimization                                                                           & Performance optimization, conformance checks                                                                                                                                          \\
%\textbf{Enablers}                & 
%Simulations of structural analysis, uncertainity / FEM / damage
% & Simulator and machine learning component
% & Simulations of performance and forces, automated monitoring system
%\\\midrule
%%& Matlab/Simulink Models, FMI interface                                                                                                                  & Web Application, Social Network                                                                                                                                                                                        & the electromechanical model of the system an model of the P-PI cascade controller      & Information Databases, Real-time data manipulation infrastructure                                                                                                                     \\
%\textbf{Models and Data}
% & Real-time sensor data, maintenance records, damage /physical models
% & Component models, vibration data, neural network
% & Real-time sensor data, hyradulic and mechanical models  
%\\\midrule
%% & graphical representation of systems status, real-time simulation data of any signal, data analytics and aggregated data of signals, weather indicators & Battery voltage/load, Water temp., Weather \& sea conditions,  Fuel level, Range, Speed, Hull stress, GPS, Position, Temp., Humidity, Maintenance status,  Maintenance offers, Upgrade offers, Usage hints \& warnings & Measured physical and electrical parameter values, optimized control  parameter values & ground plan, layout, purpose of the production machine, parts list, qualification of employees, shifts, production flow, movements of employees, machine assignment, transport routes \\
%%
%\textbf{Slices}
% & Not explicit
% & Not explicit
% & Not explicit   
%\\  \midrule
%%& Design and maintenance, storage and upgrades, process monitoring                                                                                                                                                       & not explicit                                                                           & not explicit                                                                                                                                                                          \\
%%\textbf{Fidelity Considerations} & Ultra-precise fid. req. for both usages                                                                                                                                                                                 & Realistic forces and modelling req.                                                           & Realistic data and modelling
%%& unclear                                                                                                                                                & unlcear                                                                                                                                                                                                                & high                                                                                   & unclear                                                                                                                                                                               \\
%\textbf{Data Communicated}
% & Load data, flight parameters           
% & Vibration, speed, power output
% & Temperature, pressure, etc.
%\\\midrule
%%& unclear                                                                                                                                                & sensor data, owner interactions                                                                                                                                                                                        & not explicit                                                                           & sensor and camera data from equipment to DT                                                                                                                                           \\
%\textbf{Insights / Actions}
% & Life expectancy and damage prediction reports                         
% & Maintenance insights
% & Drill control signals, performance reports
%\\\midrule
%%& unclear                                                                                                                                                & unclear                                                                                                                                                                                                                & Optimizing control parameters                                                          & unclear                                                                                                                                                                               \\
%\textbf{Time-Scale}
% & Real-time for sensor data, slower-t-r-t for health data reports
% & Real-time data, slower-t-r-t for health data reports for maintenance insights
% & Real-time for control, slower-t-r-t for reports/training, faster-t-r-t for sim.(?)
%\\\midrule
%%& slower than realtime                                                                                                                                   & Real-time, slower than realtime                                                                                                                                                                                        & slower than real time                                                                  & Real-time, slower than real-time                                                                                                                                                      \\
%\textbf{Actuators}
% & None (no actions)
% & None (no actions)
% & Not explicit
%\\\midrule
%%& None                                                                                                                                                & None                                                                                                                                                                                                                & None                                                                                & None                                                                                                                                                                               \\
%\textbf{Sensors}
% & Vehicle sensors
%%damage sensing data, performance data, structural integrity, temperature
% & Speed, vibration, power sensors
% & Operational sensors
%
%\\\midrule
%%                                     & undefined                                                                                                                                              & GPS, temperature, fuel, etc.                                                                                                                                                                                           & unclear                                                                                & timers, cameras, motion detectors                                                                                                                                                     \\
%\textbf{Life-cycle Stage}
% & Utilization
% & Utilization
% & Ideation, realization, utilization
%\\\midrule
%%& ideation, realization                                                                                                                                  & utilization                                                                                                                                                                                                            & ideation, realization                                                                  & utilization                                                                                                                                                                           \\
%\textbf{Evolution}
% & Not reported 
% & Not reported
% & Used for training, then used for control(?)
%\\\bottomrule
%%& unclear                                                                                                                                                & unclear                                                                                                                                                                                                                & unclear                                                                                & unclear                                                                                                                                                                            
%\end{tabulary}

\end{table*}}
%\end{landscape}



%\normalsize

==> sections/further_examples.tex <==
\section{APPLICATION EXAMPLES}
\label{sec:further_examples}

This section examines four selected works from the literature described as digital twins (DTs), using our conceptual structure to produce a table of characteristics (\cref{tab:further_examples}). This section is to demonstrate applicability to DT solutions in multiple domains, and highlight how this structure ensures that these characteristics are reported to assist with further classification and insights. As a visual guide, missing entries are marked in bold, while unclear information is marked in italics. Similar to \cref{sec:key_char}, only the briefest of details are reported here due to space considerations. 

%. Any missing or unclear information can affect the ease of classification of the solution and thus hamper

%motivating our framework which provides a structure of DT components and a checklist of the DT characteristics to report in future case studies.

\input{sections/further_example_table}


\emphtwo{Boat Avatar}
\cite{Wuest2015} describe a ``product avatar'' approach where the information from sensors on leisure boats is used to provide services to manufacturers and boat owners. For example, maintenance information is collected during the winter season when boats are in storage, and service offers are relayed to service providers and boat owners to offer repairs or refurbishment.

\cite{Uhlenkamp2019} identifies this experience report as a ``digital twin application scenario''. However, this report is difficult to classify according to \cite{Kritzinger2018} as it mostly describes a \textit{digital shadow} where no automatic actions are commanded. We have identified one possible action: boat information could be automatically posted to social networks. Further clarification by the authors is therefore required to classify the DT solution as a \textit{digital twin}.% as per \cite{Kritzinger2018}.

As well, it is difficult to understand the precise system-under-study (SUS), insights, and actions involved. In particular, in \cref{tab:further_examples} we have placed the boat manufacturers and the boat owners as \textit{agents} and as part of the SUS, but this may not be the intention of the report authors.

\emphtwo{Cyber Guided Vehicle}
\cite{Bottani2017} detail the creation of a simulation for an Automated Guided Vehicle (AGV) in the context of a job-shop where the AGV transports materials to be assembled. The same code from the AGV runs inside the simulation, which is used to optimize the AGV's policies for maximum profit.

This report also lacks relevant details about the DT solution. In particular, Table~1 in \cite{Kritzinger2018} claims that this solution is a \textit{digital twin}. However, from our reading the only communication between the digital object and the physical AGV would be the policies or AGV code. It is unclear whether this communication would be automatic to and from the AGV to the digital object and how often this would occur. This experience report may thus describe a \textit{digital shadow}.
%, and therefore whether most practitioners would consider this to be a ``true'' DT

%\emphtwo{Wind Turbine Gearbox}
%Tao \textit{et al.} build a solution for monitoring the health of wine turbine gearboxes, and suggesting repair operations~\cite{Tao2018a}. Live data from the gearboxes is collected and examined to determine if there has been a fault, or if performance is degraded. If an issue is present, a repair strategy is simulated and then issued for the physical gearbox.
%
%This experience report is a prime example of a \textit{digital shadow}, where the real-time data is communicated from the system-under-study and maintenance insights are delivered back for manual implementation. Our framework therefore highlights these insights as a prime candidate for implementation as automatic actions, which would promote this solution to the  \textit{digital twin} classification.

\emphtwo{Oil and Gas Drilling}
\cite{Mayani2018}~report the successes of using DT technology by a Norwegian oil and gas technology provider. Four uses of the DT technology at three oil and gas wells for monitoring and training purposes are discussed, as well as the cost- and time-saving benefits. As drill parameters are optimized based on the digital object, the overall solution is a \textit{digital twin} by the classification by \cite{Kritzinger2018}. However, the training usage of the solution may not lead to automated control actions with the SUS, thus indicating that the DT solution acts as a \textit{digital shadow} for some usages.% This more nuanced classification is highlighted by the explanations required by our framework.

\emphtwo{Petrochemical Optimization}
%Data from the industrial Internet of Things (IoT) is connected to the DT from factory sensors.
\cite{Min2019} provide an excellent report on the use of digital twins for optimization of petrochemical production. Data from factory sensors undergoes cleaning such as time series unification, before it is used alongside historical data for machine learning training and prediction. The DT solution determines recommendations and control actions to improve the economic potential of the plant, such as by increasing the yield of light oil.

As this report explicitly mentions the use of control actions on the plant, our reading suggests it is a \textit{digital twin} as per the classification by \cite{Fuller2019}. However, this report is classified as a \textit{digital shadow}, possibly due to the ambiguous sentence ``[the output], real-time recommended control information, is viewed by operators first before being utilized in the production system''. It is therefore not clear if the control information is presented as insights, or is an action on the system. The capabilities and classification of this DT solution would therefore be clarified when presented in our conceptual structure.

%The eDrilling technology began as mathematical models and visualizations for drilling operations, before being expanded for use in real-time diagnostics and training. Support for the planning of drilling operations was then added.

%
%%\subsection{Space Satellites}
%%
%%\cite{Dahmen2018} Not enough info here?
%
%\subsection{CAD with Visualization}
%
%\cite{Miller2018} This may not be a Digital Twin. Maybe just Digital Model or Shadow.

%\subsection{Nautical Thruster Control}
%\cite{Ludvigsen2016}
%
%Maybe just Digital Shadow, with some manual maintenance operations.

%\subsection{Air Force Examples}
%
%Wind tunnel? Look at `IV. The AF Digital Thread / Digital Twin'
%\cite{Kraft2016}
%
%\cite{Tuegel2011}
%


%
%\subsection{Optimization}
%\cite{Guerra2019}

%\subsection{Production Systems}
%\cite{Uhlemann2017}
%
%\subsection{Living Systems}
%The digital twin literature often focuses on the twinning of non-living systems such as products or factories. In the work of El Saddik, digital twins (DTs) are presented for living systems, such as the health status of a tree or as a representation of a living person after death~\cite{ElSaddik2018}. 

==> sections/motivation.tex <==

%\vspace*{-2em}
\section{MOTIVATION}
\label{sec:motivation}
%\vspace*{-1em}
This section motivates our proposed conceptual structure by examining a digital twin (DT) experience report for a ``human-robot collaborative work environment''~\cite{Malik2018}. This report was selected for its recency, industrial relevance, and complexity.

%, as discussed below after a short summary. This case study \ali{experience report} will be examined in \cref{sec:key_char} through the lens of our framework to provide examples of the characteristics present in our framework.
%
%\subsection{case study \ali{experience report} Summary}

The experience report domain is an industrial assembly process utilizing plastic and metallic parts to assemble an (unreported) product, where the production is high in volume and the diversity of variants. Assembly is performed using a human-robot collaborative system, combining the flexibility of humans with the efficiency of machines. This collaborative system is challenging however, as any changes to the process requires new analyses for potential collisions between the human and the robot, the workflow itself, and possibly the generation of new robot code.

The report suggests assistance for these analyses using a DT. The data from the factory floor such as the production requirements and inventory is provided to the DT as input. This input is then utilized for DT usages such as visualization, task allocation between humans and robots, workstation layout/ergonomic analysis, and programming the robot. Each usage is enabled through simulation of the assembly task and optimization of various parameters as defined by fitness metrics. The DT then produces workspace planning, a task allocation, and behavioural code for the robot.

%For example, the DT solution can perform a reach test for both the human and robot based on the proposed layout of the assembly workstation to ensure that both the robot and the human can safely reach all required positions without strain.

\paragraph*{Unreported Characteristics}

%The report attempts to be comprehensive, yet 
We find that essential characteristics about the DT solution are not reported in this report, and there is precision missing which would be valuable to characterize this DT and provide a basis for further research.

For example, the \textit{time-scale} of the DT solution is not clear as regards to each DT \textit{usage}. As described in \cref{sec:fw_time_scales}, the time-scale of a DT activity could be classified into \textit{slower-than-real-time}, \textit{real-time}, or \textit{faster-than-real-time} (utilizing predictive simulations). The experience report  describes real-time data flowing into the DT, however all of the DT usages are described as ``off-line''. Therefore it is not clear if the DT utilizes predictive simulations employing this real-time data as it comes in, or whether the real-time data is simply a source of metrics for the off-line simulations triggered when production parameters change. 

%For example, the lack of real-time control present in this report means that this DT does not possess the capabilities of the framework envisioned by Zhuang \textit{et al.}~\cite{Zhuang2018}.

Section~5 of the paper also mentions ``real-time performance metrics, optimization analytics and alerts for a robot'' supported by a commercial robot analysis tool. It is therefore not clear whether the DT produces \textit{insights} into the assembly workstation (such as a status dashboard) based on this real-time data, or whether it is only receiving the data for use in manually-activated simulations and optimizations.

%Further information about the \textit{evolution} of the experience report would also be relevant to DT researchers and practitioners, such as which \textit{usages} were developed first during the DT project. For example, how the DT evolves from a \textit{digital model}, through the \textit{digital shadow} stage, to become a \textit{digital twin}~\cite{Kritzinger2018}.

\paragraph*{Difficulties with Classification}

As described in the introduction, this precise information about the DT activities can be crucial for researchers and practitioners to classify the DT solutions appropriately. For example, while the DT solution in the report is discussed as a \textit{digital twin}, it is classified as a \textit{digital shadow} by \cite{Fuller2019}. They rely (as we do) on the classification of \cite{Kritzinger2018} who specify that the distinctive characteristic of a \textit{digital twin} compared to a \textit{digital shadow} is the automatic flow of information from the digital object to the physical object. In our reading of this experience report, the distinction between \textit{digital shadow} and \textit{digital twin} for this report comes down to whether there exists an automatic procedure for adaptation of controller code for the robots based on workstation conditions. If there is an \textit{automatic action} as described in \cref{sec:fw_data_insights_actions}, then their solution may yet be a \textit{digital twin}, but it is unclear from the paper whether such a procedure exists.
This omission about the characteristics and capabilities of the DT solution affects the classification by not only Fuller \textit{et al.}, but also \cite{Uhlenkamp2019} who distinguishes between manual, semi-automated, and automated \textit{data integration}. We therefore claim that having structured information about the reported DT solution would resolve this classification issue and could lead to further valuable insights into DTs. This is demonstrated in \cref{sec:key_char} by summarizing the main characteristics of this experience report.
%Authors of experience reports might omit essential characteristics of their DT solution and valuable contributions to the state-of-the-art due to lack of a clear structure for reporting their DT solution.
%In turn, researchers and practitioners will be better able to understand and classify the solution.  
%The conceptual structure in this paper thus serves as this structure for reporting, 


%Consider the optimization of the robot's movement and logistical procedure as described in Section~4.4 of the report. In this activity, the DT performs simulation and optimization of the workstation activities, resulting in generated robot code. 
%


%How many solvers/visualizors? Which models/data for training/optimization? What actions/insights exactly does the digital twin provide (alerts/optimization?/training)? What modifications were necessary to support the digital twin? How does the digital twin evolve over time (both the digital twin software, and on a job site, how does it evolve)?
%
%Real-time optimization? Or just insights?
%
%Real-time data from system always or just sometimes?



==> sections/nasa_table.tex <==
\begin{table*}[tbp]
	\caption{Digital twin characteristics and their relation to the NASA vehicle case study~\cite{Glaessgen2012}}
	\label{tab:characteristics}
	
	\begin{tabulary}{\linewidth}{L | L | L}
		\toprule
		\textbf{Character.} & \textbf{Short Desc.} & \textbf{Case Study Details}\\
		\midrule
		System-under-study & Scope of the SUS (components, influencing factors) & Aerospace vehicles, materials, external forces, vehicle records\\\midrule
		Multiplicities & How many DTs and SUSs are involved& One DT for each vehicle in the fleet (?), and one DT to manage the whole fleet (?)\\\midrule\midrule
		
		Usages & Activities the DT is used for & Anomaly detection, vehicle health, prob. of mission success\\\midrule
		Enablers & DT components to support usages & Fault tree reasoner, material simulations, mission profile manager \\\midrule
		Models and Data & Input and output for enablers & Models of materials, vehicle data, historical fleet data\\\midrule
		Slices & Relationships between usages, enablers, and models and data & Not explicitly connected in the report\\\midrule\midrule
		
		Fidelity Considerations & Explanations of fidelity of DT to SUS with respect to each DT usage & High-fidelity required wrt. physical effects for anomaly detection/health, wrt. mission parameters for prob. of mission success\\\midrule
		
		
		Data Communicated & What is transferred from the SUS to the DT& Sensor data from vehicle, fleet records\\\midrule
		Insights \& Actions & What is communicated from the DT to the SUS& Self-healing actions, changes in mission profile\\\midrule
		Time-Scale & The time-scale of the data/insights/actions & Slower-than-real-time insights for ideation usages, slower-than-real-time insights and real-time actions for utilization usages\\\midrule\midrule
		
		Actuators & Modifications to the SUS to enable the DT actions& Unclear\\\midrule
		Sensors & Modifications to the SUS to enable DT data collection & Unclear\\\midrule\midrule
		
		Life-cycle Stages & Stages of the life-cycle the DT is used in & Ideation, realization(?), and utilization\\\midrule
		Evolution & How the DT evolves over the DT project timeline & Not detailed in report\\
		
		\bottomrule
	\end{tabulary}
\end{table*}

==> sections/related.tex <==
\section{RELATED WORK}
\label{sec:related}

%This section presents a selection of the digital twin (DT) literature organized into framework definitions and the aspects and characteristics of DTs.

\subsubsection*{Structured DT Definitions}

\cite{Grieves2017} define DT Prototypes, DT Instances, and DT Aggregates. DT Prototypes exist only in the design stage of a system, before being realized as a \textit{Physical Twin}. Each Physical Twin is then monitored and acted upon by a DT Instance. A collection of DT Instances is a DT Aggregate. This structuring parallels our own, where DT Prototypes would be the models and data involved in a DT Constellation while the DT Constellation operates in the design stage of a system.  The concept of the DT Instance is the same as a particular instance of a DT communicates with a system-under-study (SUS). Our structure requests that the multiplicity of the DTs with relation to the SUS be explicit for clarity, such as whether multiple DT instances are aggregated to form a DT of a larger system.%, such as DTs for each machine in a factory.% This multiplicity precision offers clarity on the relationship between the DTs and the SUS.

%An essential classification for Digital Twins is the division between Digital Models, Digital Shadows, and Digital Twins~\cite{Kritzinger2018}. As a recap, Digital Models do not have communication with the SUS, Digital Shadows (or tracking simulators) receive data from the SUS but do not send actions, and Digital Twins both receive data and send actions. This classification has been embodied in our framework where the characteristics of the communication between the DT and the SUS must be specified. This classification allows us (and the authors of~\cite{Kritzinger2018}) to determine that some of the DT examples in the literature are not ``true'' DTs as seen in \cref{sec:further_examples}.

\cite{Tao2018a} present a five-component structure for relating DTs and the SUS: a) the \textit{physical entity model} which is the SUS including sensors and actuators, b) the \textit{virtual equipment model} including models and behaviour description, c) a \textit{services model} with the \textit{usages} of the DT and include quality information, d) a \textit{DT data model} to structure the domain knowledge of the DT, and e) a \textit{connection model} which structures the incoming or outgoing data from the DT, such as variable type and sampling interval.  In contrast, our structure is at a higher level of abstraction and is not about technical details but only a summary of the characteristics and capabilities.
%A similar framework is also proposed by \cite{Josifovska2019}.
%Another aspect not considered in their work is the \textit{evolution} aspect of DTs, where the DT is involved in different life-cycles of the system, and where usages of the DT are added or modified over time.

Further work by \cite{Tao2019} focuses on the use of DTs for product design and manufacturing, such as enabling technologies for DTs and a `V-cycle' for validating and verifying product design. Also relevant is the investigation of the steps of \textit{building} the DT for product design, which is similar to our concept of \textit{evolution}. These steps involve the creation of the virtual product and its connection with the physical product, where the DT solution moves from a \textit{digital model} through a \textit{digital shadow} stage to become a \textit{digital twin}.

\cite{Worden2020} take a mathematical approach to DTs where \textit{mirrors} are defined which replicate the behaviour of a system in an environment and context according to a fidelity measure. These \textit{Turing mirrors} must provide the same answers to questions as the original physical system. This is relevant to our work as it formalizes our \textit{fidelity} characteristic.% The other characteristics of DTs are however not examined.

%The work of \cite{Josifovska2019} describes a DT framework based on the 5-level cyber-physical systems architecture, therefore making a distinction between physical entity, virtual entity, data management, and service platforms, where the latter two handle the communication between the virtual and physical spaces. The goal of the framework is to help solidify the definition of DTs and their interrelations within the context of CPSs. They, however, do not explore what separates a DT from a digital shadow or a model.


%\cite{Fitzgerald2019} describe how the tools and methods available during the design and development of a CPS can be further refined into a DT optimized for learning. %%%% NOT REALLY RELEVANT 



\subsubsection*{Digital Twin Aspects/Characteristics}

\cite{Boschert2016} discuss the use of DTs for simulation throughout a system's life-cycle stages and the need for DTs to be modular to fit into \textit{value chains}. The DT \textit{purpose} may also change due to the current life-cycle stage of the system or the maturity of the DT itself.

Similar to our work, \cite{Uhlenkamp2019} present seven characteristics of DTs. 
\textit{Goals} refer to the abilities of the DT and include \textit{information acquisition}, \textit{information analysis}, \textit{decision and action selection} and \textit{action implementation}. \textit{Users} focus on one user or multiple stakeholders. \textit{Life-cycle focus} can likewise be a single stage or multiple. A \textit{system focus} can be \textit{component}, \textit{subsystem}, \textit{system}, or \textit{system of systems}. \textit{Data sources} for a DT include \textit{measurements}, \textit{virtual data} (including simulation data), and (expert) \textit{knowledge}. \textit{Data integration levels} replace the classification of \cite{Kritzinger2018} with \textit{manual}, \textit{semi-automated}, and \textit{automated}. Finally, their characteristics include \textit{authenticity} which we refer to in our conceptual structure as \textit{fidelity}. While relevant, we demonstrate in \cref{sec:motivation} that further characteristics and detail may be required in current experience reports to apply their structure. %This lack of required detail thus motivates our framework with additional structure and characteristics.

According to \cite{Madni2019}, DTs are an enabling technology in the next steps of \textit{model-based system engineering} (MBSE). A comprehensive examination of DTs within the context of MBSE is presented, along with a classification of DT maturity throughout the life-cycle of the system of \textit{pre-DT}, \textit{DT}, \textit{adaptive DT}, and \textit{intelligent DT}. Relevant to our work is a list of characteristics which separates DT from traditional \textit{computer-assisted design} (CAD) models, including \textit{specificity}, \textit{understanding assumptions and performance}, and \textit{traceability} among others. 

%For deployment of DTs into systems such as production systems, there are many challenges and considerations for proper integration. As an example, \cite{Uhlemann2017} discuss the steps for incrementally building and integrating a DT for production systems in \textit{small and medium enterprises} (SMEs). For example, sensor tracking and machine learning can be used to obtain new data for the DTs instead of focusing on the standardization of data in the organization's databases.

%The volume (and variety and velocity) of data required by some usages of a DT is also a concern~\cite{Qi2018}, such as information on product design, manufacturing, transportation, sales, and usage~\cite{Tao2018}. As high amounts of data is generated throughout the life-cycle of a system, specialized \textit{big data} techniques are required to ensure that the data is efficiently acquired, processed, and stored to enable DT usages.

%The DT literature often focuses on the twinning of non-living systems such as products or factories. In the work of El Saddik, DTs are presented for living systems, such as the health status of a tree or as a representation of a living person after death~\cite{ElSaddik2018}. In this framework, these DTs have several characteristics such as \textit{sensors and actuators}, \textit{artificial intelligence (AI)}, \textit{communication} with their environment and real twins, \textit{trust} such that a real twin can trust a DT, and \textit{privacy and security} to protect the real twin's data.

%\cite{Tekinerdogan2020}


%\cite{Wagg2020a} %%%% seems not too relevant, more on the physical aspect.

\cite{Valk2020} propose a DT taxonomy with characteristics and relationships, while \cite{Jones2020} details a literature survey. These works propose further characteristics of DTs, but do not create a conceptual structuring.

% While similarities exists between their discovered taxonomy and our framework, theirs is mostly focused on the relation between a DT and a physical entity and lacks the conceptual formalization of a DT framework.
%
%
% extracting the most common characteristics and use-cases of DTs, and creating a mapping between them. Several of these characteristics are similar to our DT framework, however, Jones \etal stop short of fitting these characteristics within a coherent conceptual framework. 

